Mega-TTS 2: Boosting Prompting Mechanisms for Zero-Shot Speech Synthesis

Zero-shot text-to-speech (TTS) aims to synthesize voices with unseen speech prompts, which significantly reduces the data and computation requirements for voice cloning by skipping the fine-tuning process. However, the prompting mechanisms of zero-shot TTS still face challenges in the following aspects: 1) previous works of zero-shot TTS are typically trained with single-sentence prompts, which significantly restricts their performance when the data is relatively sufficient during the inference stage. 2) The prosodic information in prompts is highly coupled with timbre, making it untransferable to each other. This paper introduces Mega-TTS 2, a generic prompting mechanism for zero-shot TTS, to tackle the aforementioned challenges. Specifically, we design a powerful acoustic autoencoder that separately encodes the prosody and timbre information into the compressed latent space while providing high-quality reconstructions. Then, we propose a multi-reference timbre encoder and a prosody latent language model (P-LLM) to extract useful information from multi-sentence prompts. We further leverage the probabilities derived from multiple P-LLM outputs to produce transferable and controllable prosody. Experimental results demonstrate that Mega-TTS 2 could not only synthesize identity-preserving speech with a short prompt of an unseen speaker from arbitrary sources but consistently outperform the fine-tuning method when the volume of data ranges from 10 seconds to 5 minutes. Furthermore, our method enables to transfer various speaking styles to the target timbre in a fine-grained and controlled manner. Audio samples can be found in https://boostprompt.github.io/boostprompt/.

==> sections/_1_unused_parts.tex <==
% Table 1 mega2
\begin{table}[t]
\caption{The information limitation in prompt-based zero-shot TTS synthesis.}
\label{table_1}
\centering
\begin{tabular}{@{}c|c|c@{}}
\toprule
Speaking Style & Information Required & Prompt length required\\ 
\midrule
Identity & Voice identity & Short prompt\\
Pronunciation & Distinction of vowels, consonants, and stress & Longer prompt\\
Prosody & Intonation, stress, and rhythm & Longer prompt \\
\bottomrule
\end{tabular}
\end{table}

% Table dataset mega2
\begin{table}[t]
\label{table:dataset_used}
\caption{Datasets used to train Mega-TTS 2. ``Clips'' and ``Phoneme Tokens'' refer to the number of speech clips and phoneme tokens, respectively.}
\label{table_dataset_config}
\centering
\begin{tabular}{@{}l|cccc@{}}
\toprule
\bfseries Datasets & \bfseries Clips & \bfseries Phoneme Tokens & \bfseries Duration (hours)\\      
\midrule
GigaSpeech~\citep{chen2021gigaspeech} & 8.1M & 396.9M & 9.6k\\
LibriLight~\citep{kahn2020libri} & 10.0M & 652.3M & 17.9k\\
LibriTTS~\citep{zen2019libritts} & 375.1k & 23.6M & 573.2\\
\midrule
WenetSpeech~\citep{zhang2022wenetspeech} & 14.0M & 325.5M & 9.3K \\
AISHELL-3~\citep{shi2020aishell} & 88.0k & 2.2M & 85.0 \\
Didi 500~\citep{guo2021didispeech} & 52.0k & 1.6M & 60.2 \\
AIDataTang & 237.3k & 5.3M & 198.5 \\
MagicData & 609.6k & 14.2M & 750.0 \\
ST-CMDS & 102.6k & 2.5M & 109.0 \\
\bottomrule
\end{tabular}
\end{table}




